Using a hierarchy of Domain Specific Languages in complex software systems design

A new design methodology is introduced, with some examples on building Domain Specific Languages hierarchy on top of Scheme.

==> xZ0art.tex <==
\begin{ZZZZschemedisplay}%
(\=(\va{RESULT} \va{anyresult}) \va{unparsed-input-rest})\\%
 \>\sy{or}\\%
((\va{FAIL} \va{reason}) \va{input})
\end{ZZZZschemedisplay}


==> xZ10art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} ($p^{OR^0}$ $p_1$ $p_2$)\\%
\PRN `\=($\lambda$ (\cn{l})\\%
  \>\PRN \=(\cn{let} \=(($r_1$ (,$p_1$ \cn{l})))\\%
  \> \>     \>\PRN \=(\cn{if} \=(\cn{success?} $r_1$)\\%
  \> \>     \> \>    \>\PRN \=$r_1$\\%
  \> \>     \> \>    \> \>(,$p_2$ \cn{l})))))
\end{ZZZZschemedisplay}


==> xZ11art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} ($p^{OR}$ $p_1$ . $\vec{p_o}$)\\%
\PRN `(\cn{pselect} $p^{OR^0}$ ,$p_1$ ,{\atsign}$\vec{p_o}$))
\end{ZZZZschemedisplay}


==> xZ12art.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define} \va{parse-num}\\%
\PRN \HL \=($p^+$\\%
  \>\PRN \HL \=($p^{OR}$ \=(\va{pcsx-or} (\dt{\#$\backslash$$-$} \dt{\#$\backslash$$+$}))\\%
  \>  \>     \>\va{parse-any})\\%
  \>  \>(\va{pMANY} \va{pdigit})\\%
  \>  \>($p^{OR}$ \=($p^+$ \=(\va{pcharx} \dt{\#$\backslash$.})\\%
  \>  \>     \>    \>(\va{pMANY} \va{pdigit}))\\%
  \>  \>     \>\va{parse-any})))
\end{ZZZZschemedisplay}


==> xZ13art.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define} \va{parse-num}\\%
\PRN \HL \HL \=(\va{regexp}\\%
   \>\PRN \HL \=((\dt{\#$\backslash$$-$} \va{/} \dt{\#$\backslash$$+$}) \va{/} \va{parse-any}) \va{$+$} \\%
   \>  \>\PRN \=(\va{pdigit} \va{$\ast$}) \va{$+$}\\%
   \>  \> \>((\dt{{\tt\dq}.{\tt\dq}} \va{$+$} (\va{pdigit} \va{$\ast$})) \va{/} \\%
   \>  \> \>\va{parse-any})))
\end{ZZZZschemedisplay}


==> xZ14art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} (\va{exp1} . \va{v})\\%
\PRN \=(\va{defparsers}\\%
 \>\PRN \=(\sy{letrec}\\%
 \> \>\PRN \=((\va{epr}\\%
 \> \> \>\PRN \PRN \=(\sy{let}\\%
 \> \> \>  \>\PRN \=((\va{body}\\%
 \> \> \>  \> \>\PRN \PRN \=(\va{regexp}\\%
 \> \> \>  \> \>  \>\PRN \=(\va{num} \dt{:$-$$\gt$} ${}^\$0$) \va{/}\\%
 \> \> \>  \> \>  \> \>(\va{lst} \va{-$\gt$} (\va{aprs} \va{epr})))))\\%
 \> \> \>  \> \>(\va{regexp}\\%
 \> \> \>  \> \>\PRN \=((\va{body} \va{$+$} (\va{SCM} \va{psym} \va{$+$}) \va{$+$} \va{epr})\\%
 \> \> \>  \> \> \>\PRN \dt{:$-$$\gt$} (\va{list} (\va{$+$} ${}^\$0$ ${}^\$2$))) \va{/}\\%
 \> \> \>  \> \> \>((\va{body} \va{$+$} (\va{SCM} \va{psym} $-$) \va{$+$} \va{epr})\\%
 \> \> \>  \> \> \>\PRN \dt{:$-$$\gt$} (\va{list} ($-$ ${}^\$0$ ${}^\$2$))) \va{/}\\%
 \> \> \>  \> \> \>((\va{body} \va{$+$} (\va{SCM} \va{psym} \va{$\ast$}) \va{$+$} \va{epr})\\%
 \> \> \>  \> \> \>\PRN \dt{:$-$$\gt$} (\va{list} (\va{$\ast$} ${}^\$0$ ${}^\$2$))) \va{/}\\%
 \> \> \>  \> \> \>((\va{body} \va{$+$} (\va{SCM} \va{psym} \va{/}) \va{$+$} \va{epr})\\%
 \> \> \>  \> \> \>\PRN \=\dt{:$-$$\gt$} (\va{list} (\va{/} ${}^\$0$ ${}^\$2$))) \va{/} \va{body}\\%
 \> \> \>  \> \> \> \>))))\\%
 \> \> \>(\va{car} (\va{result} (\va{epr} \va{v}))))))
\end{ZZZZschemedisplay}


==> xZ15art.tex <==
\ZZZZschemecodeintext
\va{exp1}%
\endZZZZschemecodeintext


==> xZ16art.tex <==
\begin{ZZZZschemedisplay}%
\HL (\va{exp1} \dt{5} \va{$+$} ((\dt{10} \va{/} \dt{2})$-$(\dt{1} \va{/} \dt{5})))
\end{ZZZZschemedisplay}


==> xZ17art.tex <==
\ZZZZschemecodeintext
\va{regexp}%
\endZZZZschemecodeintext


==> xZ1art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} (\va{success?} \va{r})\\%
\PRN \HL `(\cn{not} (\cn{eq?} (\cn{caar} ,\va{r}) '\cn{FAIL})))
\end{ZZZZschemedisplay}


==> xZ2art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} (\va{result} \va{r})\\%
\PRN \HL `(\cn{cdar} ,\va{r}))
\end{ZZZZschemedisplay}


==> xZ3art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} (\va{rest} \va{r})\\%
\PRN \HL `(\cn{cdr} ,\va{r}))
\end{ZZZZschemedisplay}


==> xZ4art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} (\va{parser} \va{p})\\%
\PRN \HL `\=($\lambda$ (\cn{l})\\%
   \>\PRN \=(\cn{if} \=($\emptyset?$ \cn{l}) '((\cn{FAIL} \dt{{\tt\dq}EMPTY{\tt\dq}}))\\%
   \> \>    \>\PRN (,\va{p} \cn{l}))))
\end{ZZZZschemedisplay}


==> xZ5art.tex <==
\ZZZZschemecodeintext
(\va{m} $p_1$ (\va{m} $p_2$ {\dots} (\va{m} $p_x$ $p_n$)))%
\endZZZZschemecodeintext


==> xZ6art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} (\va{pselect} \va{m} $p_1$ . $\vec{p_o}$)\\%
\PRN \=(\sy{if} \=($\emptyset?$ $\vec{p_o}$) $p_1$\\%
 \>    \>(\sy{let} \=(($p_2$ (\va{car} $\vec{p_o}$))\\%
 \>    \>     \>\PRN ($p_x$ (\va{cdr} $\vec{p_o}$)))\\%
 \>    \>\HL `(,\va{m} ,$p_1$ (\cn{pselect} ,\va{m} ,$p_2$ ,{\atsign}$p_x$)))))
\end{ZZZZschemedisplay}


==> xZ7art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} ($p^{+0}$ $p_1$ $p_2$)\\%
\PRN `\=($\lambda$ (\cn{l})\\%
  \>\PRN \=(\cn{let} (($r_1$ (,$p_1$ \cn{l})))\\%
  \> \>\PRN \=(\cn{if} (\cn{success?} $r_1$)\\%
  \> \> \>\PRN \=(\cn{let} (($r_2$ (,$p_2$ (\cn{rest} $r_1$))))\\%
  \> \> \> \>\PRN \=(\cn{if} \=(\cn{success?} $r_2$)\\%
  \> \> \> \> \>    \>(\cn{cons} \=(\cn{cons} '\cn{RESULT} \\%
  \> \> \> \> \>    \>      \>\PRN \HL \=(\cn{append} \\%
  \> \> \> \> \>    \>      \>  \>\PRN \HL \=(\cn{result} $r_1$) \\%
  \> \> \> \> \>    \>      \>  \>  \>(\cn{result} $r_2$)))\\%
  \> \> \> \> \>    \>      \>(\cn{rest} $r_2$))\\%
  \> \> \> \> \>    \>(\cn{cons} (\cn{list} '\cn{FAIL} \dt{{\tt\dq}p$+${\tt\dq}} (\cn{car} $r_2$)) \cn{l})))\\%
  \> \> \> \>$r_1$))))
\end{ZZZZschemedisplay}


==> xZ8art.tex <==
\begin{ZZZZschemedisplay}%
(\va{define-macro} ($p^+$ $p_1$ . $\vec{p_o}$)\\%
\PRN \HL `(\cn{pselect} $p^{+0}$ ,$p_1$ ,{\atsign}$\vec{p_o}$))
\end{ZZZZschemedisplay}


==> xZ9art.tex <==
\ZZZZschemecodeintext
\va{pselect}%
\endZZZZschemecodeintext

